"Knowing When You Don't Know": A Multilingual Relevance Assessment Dataset for Robust Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) grounds Large Language Model (LLM) output by leveraging external knowledge sources to reduce factual hallucinations. However, prior work lacks a comprehensive evaluation of different language families, making it challenging to evaluate LLM robustness against errors in external retrieved knowledge. To overcome this, we establish NoMIRACL, a human-annotated dataset for evaluating LLM robustness in RAG across 18 typologically diverse languages. NoMIRACL includes both a non-relevant and a relevant subset. Queries in the non-relevant subset contain passages judged as non-relevant, whereas queries in the relevant subset include at least a single judged relevant passage. We measure relevance assessment using: (i) hallucination rate, measuring model tendency to hallucinate, when the answer is not present in passages in the non-relevant subset, and (ii) error rate, measuring model inaccuracy to recognize relevant passages in the relevant subset.In our work, we observe that most models struggle to balance the two capacities. Models such as LLAMA-2 and Orca-2 achieve over 88% hallucination rate on the non-relevant subset. Mistral and LLAMA-3 hallucinate less but can achieve up to a 74.9% error rate on the relevant subset. Overall, GPT-4 is observed to provide the best tradeoff on both subsets, highlighting future work necessary to improve LLM robustness. NoMIRACL dataset and evaluation code are available at: https://github.com/project-miracl/nomiracl.

==> tables/nomiracl_examples_non_valid.tex <==
\begin{table*}[t!]
    \resizebox{\textwidth}{!}{\begin{tabular}{l  l  c  c }
        \toprule
        \multicolumn{1}{l}{\textbf{Language}}    &
        \multicolumn{1}{c}{\textbf{Query}}   &
        \multicolumn{1}{c}{\textbf{Judged Passages}} & \multicolumn{1}{c}{\textbf{Relevance}} \\ \midrule
   \rowcolor{red!15} English (\texttt{en}) & \multicolumn{1}{p{3cm}}{What is the name of the winner of the Abel Prize of 2022?} & \multicolumn{1}{p{19cm}}
   {[1] \textbf{Abel Prize}: The Abel Prize () is a Norwegian prize awarded annually by the King of Norway to one or more outstanding mathematicians. It is named after Norwegian mathematician Niels Henrik Abel (1802–1829) and directly modeled after the Nobel Prizes. It comes with a monetary award of 6 million Norwegian kroner (NOK) (€635,000 or \$740,000).} & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[2] \textbf{MIT Department of Mathematics}: The current faculty of around 50 members includes Wolf Prize winner Michael Artin, Abel Prize winner Isadore Singer, and numerical analyst Gilbert Strang. } & 0 \\  \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[3] \textbf{Abel Prize}: After interest in the concept of the prize had risen in 2001, a working group was formed to develop a proposal, which was presented to the Prime Minister of Norway in May. In August 2001, the Norwegian government announced that the prize would be awarded beginning in 2002, the two-hundredth anniversary of Abel's birth. Atle Selberg received an honorary Abel Prize in 2002, but the first actual Abel Prize was awarded in 2003.} & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[4] \textbf{Abel Prize}: The prize was first proposed in 1899, to be part of the celebration of the 100th anniversary of Niels Henrik Abel's birth in 1902. Shortly before his death in 1899, the Norwegian mathematician Sophus Lie proposed establishing an Abel Prize when he learned that Alfred Nobel's plans for annual prizes would not include a prize in mathematics. King Oscar II was willing to finance a mathematics prize in 1902, and the mathematicians Ludwig Sylow and Carl Størmer drew up statutes and rules for the proposed prize. However, Lie's influence waned after his death, and the dissolution of the union between Sweden and Norway in 1905 ended the first attempt to create an Abel Prize. } & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[5] \textbf{Eötvös Loránd University}: Eötvös Loránd University (, ELTE) is a Hungarian public research university based in Budapest. Founded in 1635, ELTE is one of the largest and most prestigious public higher education institutions in Hungary. The 28,000 students at ELTE are organized into eight faculties, and into research institutes located throughout Budapest and on the scenic banks of the Danube. ELTE is affiliated with 5 Nobel laureates, as well as winners of the Wolf Prize, Fulkerson Prize and Abel Prize, the latest of which was Abel Prize winner Endre Szemerédi in 2012. } & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[6] 
   \textbf{Abel Prize}: Anyone may submit a nomination for the Abel Prize, however, self-nominations are not permitted. The nominee must be alive; however, if the awardee dies after being declared as the winner, the prize will be awarded posthumously.} & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[7] \textbf{Abel Prize}: The Norwegian Academy of Science and Letters declares the winner of the Abel Prize each March after recommendation by the Abel Committee, which consists of five leading mathematicians. Both Norwegians and non-Norwegians may serve on the Committee. They are elected by the Norwegian Academy of Science and Letters and nominated by the International Mathematical Union and the European Mathematical Society. The committee is of 2018 chaired by Norwegian mathematician Hans Munthe-Kaas (University of Bergen), and was before that, headed by Professor John Rognes.} & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15}  \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[8] \textbf{Hans Munthe-Kaas}: Munthe-Kaas received Exxon Mobil Award for best PhD at NTNU, 1989, and the Carl-Erik Frōberg Prize in Numerical Mathematics 1996 for the paper \"Lie–Butcher theory for Runge–Kutta Methods\". Munthe-Kaas is elected member of the Norwegian Academy of Science and Letters, the Royal Norwegian Society of Sciences and Letters and the Norwegian Academy of Technological Sciences. Munthe-Kaas is the chair of the international Abel prize committee (2018-2022), he is President of the Scientific Council of Centre International de Mathématiques Pures et Appliquées (CIMPA) (2017–present) and he is Editor-in-Chief of Journal Foundations of Computational Mathematics (2017–present). Munthe-Kaas was secretary of Foundations of Computational Mathematics (2005–2011) and member of the Board of the Abel Prize in Mathematics (2010–2018). } & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[9] \textbf{Science and technology in Hungary}: Among Hungary's numerous research universities, the Eötvös Loránd University, founded in 1635, is one of the largest and the most prestigious public higher education institutions in Hungary. The 28,000 students at ELTE are organized into eight faculties, and into research institutes located throughout Budapest. ELTE is affiliated with 5 Nobel laureates, as well as winners of the Wolf Prize, Fulkerson Prize and Abel Prize, the latest of which was Abel Prize winner Endre Szemerédi in 2012. } & 0 \\ \noalign{\vskip 1.5ex}
   \rowcolor{red!15} \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{p{19cm}}
   {[10] \textbf{Abel Prize}: The Abel Prize's history dates back to 1899, when its establishment was proposed by the Norwegian mathematician Sophus Lie when he learned that Alfred Nobel's plans for annual prizes would not include a prize in mathematics. In 1902 King Oscar II of Sweden and Norway indicated his willingness to finance a mathematics prize to complement the Nobel Prizes, but the establishment of the prize was prevented by the dissolution of the union between Norway and Sweden in 1905. It took almost a century before the prize was finally established by the Government of Norway in 2001, and it was specifically intended \"to give the mathematicians their own equivalent of a Nobel Prize.\" The laureates are selected by the Abel Committee, the members of which are appointed by the Norwegian Academy of Science and Letters. } & 0 \\ \noalign{\vskip 1.5ex}
   \bottomrule
    \end{tabular}}
    \caption{Randomly sampled example of a query and 10 judged passages in English (\texttt{en}) from the \textbf{non-relevant} subset (test split) in \nomiracl. Titles of each passage are marked in \textbf{bold}. The relevance judgment has been annotated manually by a native speaker.}
    \label{tab:examples_non_valid}
\end{table*}

==> tables/nomiracl_mistakes_non_valid.tex <==
\begin{table*}[t!]
    \resizebox{\textwidth}{!}{\begin{tabular}{l  l  c  c }
        \toprule
        \multicolumn{1}{l}{\textbf{Language}}    &
        \multicolumn{1}{c}{\textbf{Query}}   &
        \multicolumn{1}{c}{\textbf{Passage}} & \multicolumn{1}{c}{\textbf{Relevance}} \\ \midrule
   English (\texttt{en}) & \multicolumn{1}{p{3cm}}{When was The Global Marshall Plan Initiative formed?} & \multicolumn{1}{p{19cm}}
   {[3] \textbf{Global Marshall Plan Initiative}: As the world increasingly finds itself in a difficult, unsustainable situation as a result of rapid globalization, both in terms of environmental issues, poverty and unequal distribution, as well as the disproportionate cultural balance, \textbf{on 16 May 2003 representatives from 16 civil society organizations revived the original idea for a global Marshall Plan} as a movement for world peace, sustainability and justice, and at the Frankfurt airport, the Global Marshall Plan initiative was launched. Since the initiative should be organized as a network, i.e. locally and without hierarchies, the coordination of tasks and activities was assigned to different people and institutions: the coordination of content was taken up by Prof. Dr. Franz-Josef Radermacher as Head of FAW/n, politicians, and Josef Riegler, with particular importance on an EU level and the Eco-Social Forum Europe. The coordination, initiation and promotion of supporters’ activities internationally were assigned the Global Contract Foundation and Frithjof Finkbeiner. Due to the enormous positive response and the wide range of activities, this commission was soon transferred to the Global Marshall Plan Foundation.} & 1 \\ \noalign{\vskip 1.5ex}
   English (\texttt{en}) & \multicolumn{1}{p{3cm}}{When was Sweden founded?} & \multicolumn{1}{p{19cm}}
   {[8] \textbf{Sweden}: \textbf{An independent Swedish state emerged during the early 12th century}. After the Black Death in the middle of the 14th century killed about a third of the Scandinavian population, the Hanseatic League threatened Scandinavia's culture, finances and languages. This led to the forming of the Scandinavian Kalmar Union in 1397, which Sweden left in 1523. When Sweden became involved in the Thirty Years War on the Reformist side, an expansion of its territories began and eventually the Swedish Empire was formed. This became one of the great powers of Europe until the early 18th century. Swedish territories outside the Scandinavian Peninsula were gradually lost during the 18th and 19th centuries, ending with the annexation of present-day Finland by Russia in 1809. The last war in which Sweden was directly involved was in 1814, when Norway was militarily forced into personal union. Since then, Sweden has been at peace, maintaining an official policy of neutrality in foreign affairs. The union with Norway was peacefully dissolved in 1905. Sweden was formally neutral through both world wars and the Cold War, albeit Sweden has since 2009 openly moved towards cooperation with NATO.} & 1 \\ \noalign{\vskip 1.5ex}
   English (\texttt{en}) & \multicolumn{1}{p{3cm}}{When did Keith Windschuttle write Unemployment?} & \multicolumn{1}{p{19cm}}
   {[2] \textbf{Keith Windschuttle}: \textbf{Major published items include \"Unemployment\"} (1979), which analysed the economic causes and social consequences of unemployment in Australia and advocated a socialist response; \"The Media: a New Analysis of the Press, Television, Radio and Advertising in Australia\" (1984), on the political economy and content of the news and entertainment media; \"The Killing of History\" (1994), a critique of postmodernism in history; \"The Fabrication of Aboriginal History: Volume One: Van Diemen's Land 1803–1847\" (2002), which accuses a number of Australian historians of falsifying and inventing the degree of violence in the past; \"The White Australia Policy\" (2004), a history of that policy which argues that academic historians have exaggerated the degree of racism in Australian history; and \"The Fabrication of Aboriginal History, Volume Three: The Stolen Generations 1881–2008\", which argues the story of the \"stolen generations\" of Aboriginal children is a myth. He was editor of \"Quadrant\" magazine 2008-2015 when he became Chair of the board and editor-in-chief. He has been the publisher of Macleay Press since 1994.} & 1 \\ \noalign{\vskip 1.5ex}
   English (\texttt{en}) & \multicolumn{1}{p{3cm}}{What is terminus non Post Quem?} & \multicolumn{1}{p{19cm}}
   {[2] \textbf{Terminus post quem}: \textbf{Terminus post quem: Terminus post quem (\"limit after which\", often abbreviated to \"TPQ\")} and terminus ante quem (\"limit before which\", abbreviated to \"TAQ\") specify the known limits of dating for events. \textbf{A \"terminus post quem\" is the earliest time the event may have happened}, and a \"terminus ante quem\" is the latest. An event may well have both a \"terminus post quem\" and a \"terminus ante quem\", in which case the limits of the possible range of dates are known at both ends, but many events have just one or the other. Similarly, terminus ad quem (\"limit to which\") is the latest possible date of a non-punctual event (period, era, etc.), while terminus a quo (\"limit from which\") is the earliest. The concepts are similar to those of upper and lower bounds in mathematics.} & 1 \\ \noalign{\vskip 1.5ex}
   \bottomrule
    \end{tabular}}
    \caption{Possible annotation mistakes from the \textbf{non-relevant} English subset.}
    \label{tab:examples}
\end{table*}
